RISE: RISC-V SoC for En/decryption Acceleration on the Edge for Homomorphic Encryption

Today edge devices commonly connect to the cloud to use its storage and compute capabilities. This leads to security and privacy concerns about user data. Homomorphic Encryption (HE) is a promising solution to address the data privacy problem as it allows arbitrarily complex computations on encrypted data without ever needing to decrypt it. While there has been a lot of work on accelerating HE computations in the cloud, little attention has been paid to the message-to-ciphertext and ciphertext-to-message conversion operations on the edge. In this work, we profile the edge-side conversion operations, and our analysis shows that during conversion error sampling, encryption, and decryption operations are the bottlenecks. To overcome these bottlenecks, we present RISE, an area and energy-efficient RISC-V SoC. RISE leverages an efficient and lightweight pseudo-random number generator core and combines it with fast sampling techniques to accelerate the error sampling operations. To accelerate the encryption and decryption operations, RISE uses scalable, data-level parallelism to implement the number theoretic transform operation, the main bottleneck within the encryption and decryption operations. In addition, RISE saves area by implementing a unified en/decryption datapath, and efficiently exploits techniques like memory reuse and data reordering to utilize a minimal amount of on-chip memory. We evaluate RISE using a complete RTL design containing a RISC-V processor interfaced with our accelerator. Our analysis reveals that for message-to-ciphertext conversion and ciphertext-to-message conversion, using RISE leads up to 6191.19X and 2481.44X more energy-efficient solution, respectively, than when using just the RISC-V processor.

==> Sections/notes.tex <==
\newpage
{\color{red}

- Use real numbers in places of floating-point numbers. --> done

- Check if we are using \hecomputing everywhere. --> done

- Check figure captions. --> done

- We say ''Our accelerator uses data-level parallelism, shares the datapath between encryption and decryption operations, adopts memory reuse and memory reordering strategies, and eliminates the need for additional on-chip memory to store twiddle factors by computing them on-the-fly. '' Check all places where we say this, and make sure we are consistent in stating all ideas and the order of the ideas. --> done 

- Check if unit/module is used for individual operation blocks. Use ``unit" throughout the paper. --> done

-Need to add a couple of sentences stating why end-to-end evaluation is important. Make this a paragraph in the evaluation instead of a subsection. --> Not required

-Need to check TVLSI arxiv posting policy and post the paper to arxiv if allowed. --> email sent
}

==> coverletter.tex <==
%\afterpage{\blankpage}
\onecolumn
\noindent Dear Reviewers and Editors, \\
%\vspace{+5.0mm}
%our architecture can be easily scaled for more specific parameter sets
A preliminary version of this work appeared in ACM/IEEE International Symposium on Low Power Electronics and Design (ISLPED) 2022~\cite{azad2022race}.
In that preliminary version, we proposed an area- and energy-efficient RISC-V SoC for en/decryption acceleration on the edge for homomorphic computation. 
A copy of our ISLPED 2022 publication~\cite{azad2022race} is included in this submission for quick reference.
There are many significant differences/extensions in this submitted manuscript as compared to the ISLPED 2022 publication~\cite{azad2022race}. 
The differences/extensions are as follows:
\vspace{+5.0mm}
\begin{enumerate}
\item To enable practical \messagetociphertext and \ciphertexttomessage conversion operations for HE on resource-constrained edge devices, one needs to overcome several memory and performance-related challenges.  
%There are several memory and performance-related challenges to overcome, to make encryption for HE on the edge devices practical. 
%In the submitted manuscript, we propose a custom-designed area- and energy-efficient RISC-V based SoC for en/decryption of data for HE. 
Therefore, our ISLPED $2022$ publication~\cite{azad2022race} proposes \race containing an area-efficient accelerator design for low-end edge devices where area is particularly constrained. 
\race reduces area overhead by using a single computation unit (Butterfly Unit) for Number Theoretic Transform (NTT) and inverse NTT (iNTT), shared datapath between encryption and decryption, memory reuse and reorder techniques, RNS partitioning, and on-the-fly computation of roots/twiddle factors. 
However, \race design has to compromise the performance efficiency to achieve this area reduction.
For example, the single computation unit used to accelerate NTT/iNTT does not provide enough performance boost to meet the requirements of less constrained high-end edge devices and many applications. 
In addition, based on the end-to-end performance analysis presented in \race for \messagetociphertext conversion operation, random error sampling also adds significantly to the \messagetociphertext conversion time.
Consequently, in this work, we present a technique to parallelize NTT computation to further improve its performance at the cost of a slight increase in area and power overhead. 
%We evaluate this performance vs. area/power trade-off to identify the optimal architectures to meet different design objectives.
We also add an efficient and lightweight error sampling unit to our accelerator design to reduce the error sampling overhead in \messagetociphertext conversion operation. 

\vspace{+5.0mm}
\item 
In this work, we propose a scalable parallel implementation of an NTT unit with multiple Butterfly Units (BFUs) to improve NTT performance.
%The scalability is enabled by parameterizing our NTT design, which can support different levels of parallelism for different scheme parameters.
To support this parallelizable NTT architecture using multiple BFUs, we need to fulfill two main requirements.
%\begin{enumerate*} 
%\item We need to provide support for multi-port memory banks to read/write multiple BFUs inputs and outputs simultaneously and 
%\item We need to enable on-the-fly computation of multiple twiddle factors to perform multiple BF operations in parallel.
%\end{enumerate*}
One is the support for multi-port memory banks: moving to a multi-port memory bank design is not an efficient solution as increasing the number of ports will quadratically increase the memory area overhead~\cite{azad2022race}. 
To reduce the memory area overhead, we still use the single port memory banks as in \race but we linearly increase the number of memory banks (smaller in size) to access multiple in/outputs as we increase the number of BFUs.
With an increase in the number of memory banks, we observe a large number of memory bank conflicts.
Therefore, we extend \race memory reorder scheme to get rid of the memory bank conflicts by resolving data dependencies. 
The second requirement is on-the-fly computation of multiple twiddle factors: \race computes the required twiddle factors on-the-fly instead of storing the precomputed values to eliminate the memory area overhead.
In this work, we use a similar approach, but we need multiple twiddle factors simultaneously for parallel BFUs. 
To this end, we introduce a separate modular multiplier to compute twiddle factors in parallel with the Butterfly operations so as to avoid stalls in the NTT computation pipeline as observed by \race.  

\vspace{+5.0mm}
\item Error samples are critical to maintaining the required security level while performing HE operations. 
However, generating these high-quality error samples is one of the bottlenecks in accelerating edge-side operations. 
\race does not accelerate error sampling, however, in this work, we accelerate error sampling as well. 
Error sampling consists of two main steps, a pseudo-random number generation (PRNG) using a true random seed and generating error samples using the pseudo-random numbers.
We equip our SoC with an efficient and lightweight implementation of PRNG and integrate it with fast binomial and uniform samplers to speed up error sampling and further accelerate \messagetociphertext conversion operation. 

\end{enumerate}
\vspace{0.25in}
\noindent Sincerely,\\
Zahra Azad, Guowei Yang, Rashmi Agrawal, Daniel Petrisko, Michael Taylor and Ajay Joshi\\
Contact author: Zahra Azad (zazad@bu.edu)

